Self-Supervised Prompt Optimization

Well-designed prompts are crucial for enhancing Large language models' (LLMs) reasoning capabilities while aligning their outputs with task requirements across diverse domains. However, manually designed prompts require expertise and iterative experimentation. While existing prompt optimization methods aim to automate this process, they rely heavily on external references such as ground truth or by humans, limiting their applicability in real-world scenarios where such data is unavailable or costly to obtain. To address this, we propose Self-Supervised Prompt Optimization (SPO), a cost-efficient framework that discovers effective prompts for both closed and open-ended tasks without requiring external reference. Motivated by the observations that prompt quality manifests directly in LLM outputs and LLMs can effectively assess adherence to task requirements, we derive evaluation and optimization signals purely from output comparisons. Specifically, SPO selects superior prompts through pairwise output comparisons evaluated by an LLM evaluator, followed by an LLM optimizer that aligns outputs with task requirements. Extensive experiments demonstrate that SPO outperforms state-of-the-art prompt optimization methods, achieving comparable or superior results with significantly lower costs (e.g., 1.1% to 5.6% of existing methods) and fewer samples (e.g., three samples). The code is available at https://github.com/FoundationAgents/SPO.

==> archive/tables.tex <==
\begin{table*}[t!]
\caption{Comparison of performance between Single-Calling methods and Prompt generated by prompt optimization methods in six benchmarks. All methods are executed with GPT-4o-mini on divided test set, and we tested it three times and reported it on the average.}
\label{tab:mainres}

\renewcommand\tabcolsep{3.2pt}
\renewcommand\arraystretch{1.2}
\small
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc|cccccc}
\hline

\hline

\hline

\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{Reason Benchmarks}} & \multicolumn{6}{c}{\textbf{BBH}}  \\
& GPQA & AIME& LIAR& WSC & Negative & - & - & - & - & Avg.\\
\hline

\hline
Human & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\
IO  & 00.0 & 00.0 & 00.0 & 72.4& 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0  \\
CoT~\cite{wei2022COT} & 00.0 & 00.0 & 00.0 & 77.8& 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\
Rephrase~\cite{deng2023rephrase} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\
Step-back~\cite{hua2024step} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\ 
\hline
APE ~\cite{} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\
OPRO~\cite{yang2023large} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\
PromptAgent~\cite{xin2024prompt} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\
EvoPrompt ~\cite{} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\
PromptBreeder~\cite{chris2024pb} & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\


\rowcolor[gray]{.8}
\ours (ours) & \textbf{00.0} & \textbf{00.0} & \textbf{00.0} & \textbf{00.0} & \textbf{00.0} & \textbf{00.0} & \textbf{00.0} & \textbf{00.0} & \textbf{00.0} & \textbf{00.0}   \\
\hline

\hline

\hline

\hline
\end{tabular}
}
\end{table*}
